Fixed Parameter Tractable Linearizability Monitoring

We study the linearizability monitoring problem, which asks whether a given concurrent history of a data structure is equivalent to some sequential execution of the same data structure. In general, this problem is $\textsf{NP}$-hard, even for simple objects such as registers. Recent work has identified tractable cases for restricted classes of histories, notably unambiguous and differentiated histories. We revisit the tractability boundary from a fine-grained, parameterized perspective. We show that for a broad class of data structures -- including stacks, queues, priority queues, and maps -- linearizability monitoring is fixed-parameter tractable when parameterized by the number of processes. Concretely, we give an algorithm running in time $O(c^{k} \cdot \textsf{poly}(n))$, where $n$ is the history size, $k$ is the number of processes, and $c$ is a constant, yielding efficient performance when $k$ is small. Our approach reduces linearizability monitoring to a language reachability problem on graphs, which asks whether a labeled graph admits a path whose label sequence belongs to a fixed language $L$. We identify classes of languages that capture the sequential specifications of the above data structures and show that language reachability is efficiently solvable on the graph structures induced by concurrent histories. Our results complement prior hardness results and existing tractable subclasses, and provide a unified algorithmic framework. We implement our approach and demonstrate significant runtime improvements over existing algorithms, which exhibit exponential worst-case behavior.

==> aadt.tex <==
%!TEX root=./main.tex

\input{oodt-specs}

\section{Linearizability Monitoring for Order-Oblivious Data Types}
\seclabel{oodt-lin}

In this section, we discuss the first class of data structures which
we call order-oblivious data types or OODTs, and their
generalization $\alpha$-OODTs (where $\alpha \in \nats_{> 0}$ is a constant positive natural number),
and show that 
% This class captures a large class of data types including priority queues, counters,
% registers, and, as we show in \ucomment{Sec},
the problem of linearizability monitoring for this class is 
in the complexity class FPT,
where we treat $k$ (the number of threads) as a parameter.

\subsection{Order-Oblivious Data Types}




\myparagraph{Equivalent states}
As far as specifications are concerned, we often only care about the states of an object that are reachable.
That is, any reachable state of the object of interest can be described by some sequence in its specification.
For example, the state of a set containing two elements $[\val{1}, \val{2}]$ can be denoted as $\opr{\minsert}{\val{1}} \cdot \opr{\minsert}{\val{2}}$.
For formality, we can see `states' as equivalence classes of legal sequences. Two sequences $\tau_1, \tau_2 \in \spec_\ADT$ are considered equivalent, denoted as $\tau_1 \sim \tau_2$, if they represent the same state, that is, $\tau_1 \cdot \tau' \in \spec_\ADT \Leftrightarrow \tau_2 \cdot \tau' \in \spec_\ADT$ for all suffix $\tau' \in \opSort^*$.
For our set example, $\opr{\minsert}{\val{1}} \cdot \opr{\minsert}{\val{2}} \sim \opr{\minsert}{\val{2}} \cdot \opr{\minsert}{\val{1}}$.

In this section, we provide a generalization of a group of data types for which their histories exhibits the particular property to be anagram-agnostic. Our results show that within this group of data types, the problem of monitoring linearizability is then reduced to membership problem of an operation sequence.

\begin{definition}[Anagram-Agnostic Data Types (AADT)]\deflabel{aadt}
  A data type $\ADT$ is said to be a \emph{anagram-agnostic} if for any two anagrams $\tau_1, \tau_2 \in \spec_\ADT$, $\tau_1 \sim \tau_2$.
\end{definition}

Similar concept includes conflict-free replicated data type (CRDT) proposed by Shapiro et al.~\cite{Shapiro2011}, where concurrent updates to replicated objects are guaranteed to eventually converge.
However, Shapiro's work focuses mainly on the implementation and implication of such data types, and the characterization of CRDT is stronger than that of AADT.
Another similar concept is the notion of history independent data structures proposed by Noar et al.~\cite{Naor2001}.

We can easily see that priority queues implemented as multisets with unique priority are AADT. On the other hand, stacks and queues are not AADT as the order of insertion of values may affect the validity of their future removal.

\wrapbox{r}{
  \begin{tikzpicture}[scale=0.4]
  \drawoper{1}{4}{1}{$\enq(\val{1})$}
  \drawoper{2}{5}{2}{$\enq(\val{2})$}
  \drawoper{3}{6}{3}{$\enq(\val{3})$}
  \drawoper{7}{8}{2}{$\deq(\val{3})$}
  \end{tikzpicture}
}{\caption{Linearizable history $\hist_{\sf \pqueueDS}$
\figlabel{pq-aadt-example}}}
\myparagraph{Example}
Priority queue is a anagram-agnostic data type as its state can be determined by its contents.
Take the history $\hist_{\sf \pqueueDS} = \set{\tuple{1, \enq, \val{1}, 1, 4}, \tuple{2, \enq, \val{2}, 2, 5}, \tuple{3, \enq, \val{3}, 3, 6}, \tuple{2, \deq, \val{3}, 7, 8}}$ (Refer to \figref{pq-aadt-example}).
Reader will notice that not only is any linearization of $\hist_{\sf \pqueueDS}$ legal, it also results in a same content of $[1, 2]$, with $2$ ordered before $1$ in terms of priority.
If the same history is interpreted as a queue history, a legal linearization of the history results in a same content of $[1, 2]$, but with possibly different order, for which the order of their removal must also be different.

Reader may be inclined to think that the characterization of AADT are impractically restrictive. We argue that it is, however, not the case. 
Firstly, our characterization of AADT automatically generalizes to include any read-only operations that do not change the state of the object. For example, a priority queue supporting $\msize$ operation that retrieves the current size of the object remains an AADT.
Secondly, there are a number of ADTs, which are not anagram-agnostic by convention, that has anagram-agnostic variants that are widely studied.
Here we list out the commonly used data types that are anagram-agnostic, together with some intuition as why they are so.

\myparagraph{Counter}
Counter is the simplest AADT of all. It supports $\inc$ operation that increments the counter by 1, $\dec$ operation that decrements the counter by 1 and $\get$ operation that returns the current value of the counter. It is also easy to see that two anagrams within the counter's specification emits the same set of suffixes as the final value of the counter is always the same no matter the order in which the same set of $\inc$ and $\dec$ operations are applied.

\myparagraph{(Multi)Set/(Double-ended) Priority Queue}
(Multi)sets can be simply viewed as a set of counters, each responsible for keeping the count of the occurrences of a value within the object. Note that unlike counters, $\minsert$ and $\remove$ operations on a (multi)set object may fail (return a boolean value of $\false$) if the value is respectively already present (for sets) or absent in the object. Even for ordered sets or multisets that support order statistics queries, the final state of the object is always the same no matter how the same set of operations are ordered, and they are hence anagram-agnostic.
Since an ordered multiset can trivially simulate priority queues and double-ended priority queues with a subset of methods, we have that both priority queues and double-ended priority queues are also AADTs.

\myparagraph{Read-modify-write Register}
Perhaps surprisingly, even though register in its purest form supporting $\mread$ and $\mwrite$ operations is not anagram-agnostic, its read-modify-write variant is. We can think of a $\rmw$ operation to be an increment/decrement of the value held by the register given the pre-condition of holding specific values.
For example, $\opr{\rmw}{\val{5}}\Rightarrow\val{1}$ is an increment with a magnitude of $\val{4}$ given that the present value is $\val{1}$. Since addition/substraction is commutative, the final value of the register is always the same no matter how the operations are ordered.

\myparagraph{Size-aware Stack}
Extending the reasoning applied to read-modify-write registers, we will see that a stack that reports its size for each $\push$ and $\pop$ operation is also anagram-agnostic. One simple way to think about this is to view the stack as a really big register value $r$ initialized to the value of $1$. Say that given a stack history $\hist$, we have integer $u = \max\vals_\hist + 1$ (we assume $\vals_\hist \subset \ints^+$ for simplicity). We can then segregate each value $v$ inserted via $\push$ operation to position $i$ as an addition of value $u^{i+1} \cdot v$ given the precondition that $u^{i+1} > r \geq u^i$ holds, and likewise the substraction of the same value for $\pop$ operations. Again, since addition/substraction is commutative, the final value of the register (and hence the actual state of the stack) is always the same no matter how the operations are ordered.

\subsection{FPT Result of AADTs}

Recall from \propref{cert-general} that a general approach to construct legal linearization of a given history is to iterate through its frontier graph and compute the certification of all partition states. To circumvent the potential exponential growth in certification size, we have based on \defref{aadt} and \propref{cert-general} the following corollary:

\begin{corollary}\corlabel{cart-aadt}
  Given a history $\hist$ of an anagram-agnostic data type $\ADT$, then for all 
  \ucomment{uncomment the following after fixing `cert' and `partstate'}
  % $\tau_1, \tau_2 \in \cert{S}$, $S \in \partstate_\hist$, $\tau_1 \sim \tau_2$.
\end{corollary}

The properties of a anagram-agnostic data type presents us a notion of equivalence of linearizations within a certificate, where the derivation of just one member of the certificate suffices since it is representative of the entire certificate. This gives us the following result:

\begin{theorem}
  Given a history $\hist$ with $n$ operations of an AADT $\ADT$, where the membership of $\spec_\ADT$ can be solved in $f(n)$ time, the problem of monitoring linearizability can be solved in $O(n \log{n} + nk2^k \cdot f(n))$ time.
\end{theorem}

For many AADTs, including priority queue (interestingly)~\cite{Finkler1999}, there is a linear time procedure for solving the membership of their specifications. This automatically gives us a $O(k2^k \cdot n^2)$ time for monitoring the linearizability of the histories of these data types. Nonetheless, there is obvious room for improvements.
We can see that instead of constructing and verifying an entire sequence at each node of the frontier graph of a history, we can perform a depth-first search on this graph while maintaining a simulated state of the object.
In this way, we only have to apply one operation on the simulated object at each visitation of a node in the frontier graph.
This would, however, often require the operation to be backtrackable in an equi-efficient fashion.
The procedure can be outlined as such:

\input{algo/aadt-algo.tex}

In \algoref{aadt-lin}, we represent the $\ADT$ object state as a linearization $\lin$. As previously mentioned,
the application of operation $o$ on $\lin$ (refer to \lineref{aadt-loop-1}) may incur a relatively lower cost,
and we assume the previous state $\lin$ can be recovered equally efficiently.
This fine-grained result gives us the following:

\begin{theorem}[Linearizability Monitoring for AADTs]
  Given a history $\hist$ with $n$ operations of an AADT $\ADT$, where the initialization of the object and each operation both updates and backtracks in $O(f(n))$ time, the problem of monitoring linearizability can be solved in $O(n \log{n} + nk2^k \cdot f(n))$ time.
\end{theorem}

For example, since a priority queue can be simulated using a self-balancing binary search tree,
where each updates are (also backtrackable in) $O(\log{n})$ time,
we have that the linearizability monitoring for priority queue can be solved in $O(k2^k\cdot n\log{n})$ time.
Similarly, linearizability monitoring for hash-based (multi)sets can be solved in $O(n \log{n} + nk2^k)$ time.

While the characterisations of AADTs are extensive,
\algoref{aadt-lin} does not apply for the case of some most commonly used data types such as stacks and queues.
In the following sections, we explore interesting ways for which
the properties of stack and queue data types can be exploited
to still achieve a reasonably efficient fixed parameter tractable algorithm.


==> algo/aadt-algo.tex <==
%!TEX root=../main.tex

\begin{algorithm}
\caption{Frontier Graph $\ADT$-Reachability for AAL}
\algolabel{aadt-lin}
\myproc{$\AADTLin(G_\hist, s, t)$}
{
\Return $\DFS(E_\hist, s, t, \varepsilon, \varnothing)$
}
\;
\myproc{$\DFS(E, u, v, \tau, \visited)$}{
\lIf{$u = v$}
{ 
  \Return $\true$
}
\lIf{$u \in \visited$}
{
  \Return $\false$
}
$\visited \gets \visited \uplus \set{u}$\;
\For{$(u, \abs{o}, w) \in E$}
{
  \If{$\tau \cdot \abs{o} \in \spec_\ADT$ \AND $\DFS(E, w, v, \tau \cdot \abs{o}, \visited)$}
  {
    \linelabel{aadt-loop-1}
    \Return $\true$
  }
}
\Return $\false$
}
\end{algorithm}
